EpiKV: Epiphany-Aware KV Cache Eviction Without the Attention Matrix

Reasoning models can generate chains of thought tens of thousands of tokens long, making the key--value (KV) cache that holds them a major bottleneck for inference throughput. Existing eviction policies for long reasoning traces typically rank cached tokens using attention weights, requiring access to the attention matrix and making them incompatible with fast inference kernels. In this work we study the limits of such policies under tight cache budgets. Surprisingly, we find that under the strongest of them the generations that finish are wrong about as often as without eviction; most of the accuracy loss comes from generations that enter loops and run until the length limit, and retaining more tokens according to a fixed importance score exacerbates this behavior. What stops the looping is keeping the tokens the model's recent queries point to, and the forward pass the model already runs reveals them without the attention matrix. Motivated by this observation, we introduce epiphany-aware KV cache eviction EpiKV, which combines hidden-state shifts with the model's recent query--key relevance to rank cached tokens without materializing the attention matrix. On multiple benchmarks, EpiKV matches or outperforms the strongest attention-based eviction baselines while running directly in vLLM with unmodified attention kernels.

==> figures/pipeline_v6_mechanism.tex <==
% The method figure (bible D-5): state -> action -> state, left to right; blue marks what the
% method reads or adds, grey is the model and its cache; the toy cache in panel 3 shows the three
% compaction decisions on real segment caps (64/32/8). Drawn at the text width with real point
% sizes; never scaled. Iterated Sep 24 overnight (v6).
\vspace{-1mm}
\begin{figure}[t]
\vspace{-4mm}
\centering
\begin{tikzpicture}[x=1cm,y=1cm,font=\footnotesize,
  >={Stealth[length=1.5mm,width=1.2mm]},
  ttl/.style={font=\footnotesize\bfseries,text=ink,anchor=base west,inner sep=0},
  sub/.style={font=\scriptsize,text=mdl,anchor=base west,inner sep=0,align=left},
  box/.style={draw=mdl,fill=mdllt,rounded corners=1pt,align=center,inner sep=2.2pt,font=\scriptsize,text=ink},
  ours/.style={draw=epi,fill=epilt,rounded corners=1pt,align=center,inner sep=2.2pt,font=\scriptsize,text=ink},
  arr/.style={->,draw=mdl,line width=0.5pt},
  earr/.style={->,draw=epi,line width=0.6pt},
  cell/.style={draw=mdl!60,line width=0.3pt,minimum width=1.3mm,minimum height=3.2mm,inner sep=0,anchor=south west},
  kept/.style={cell,fill=epimid,draw=white,line width=0.4pt},
  filled/.style={cell,pattern=north east lines,pattern color=epi,draw=epi,line width=0.3pt},
]
% panel separators
\draw[mdl!35,line width=0.4pt] (2.92,-0.45) -- (2.92,3.35);
\draw[mdl!35,line width=0.4pt] (7.0,-0.45) -- (7.0,3.35);
% ============ panel 1: one decode step ============
\node[ttl] at (0,3.2) {1\;\;One decode step};
\node[sub] at (0,2.88) {unmodified FlashAttention,};
\node[sub] at (0,2.6) {no attention matrix};
\foreach \i in {0,...,6} {\draw[mdl,fill=white,line width=0.4pt] (0.45,0.3+0.3*\i) rectangle (1.65,0.5+0.3*\i);}
\def\yA{1.0}\def\yB{1.9}
\draw[epi,fill=bandA,line width=0.7pt] (0.45,\yA-0.1) rectangle (1.65,\yA+0.1);
\draw[epi,fill=bandB,line width=0.7pt] (0.45,\yB-0.1) rectangle (1.65,\yB+0.1);
\node[font=\scriptsize,text=epi,anchor=east] at (0.42,\yA) {A};
\node[font=\scriptsize,text=epi,anchor=east] at (0.42,\yB) {B};
\node[font=\scriptsize,text=mdl,anchor=north] at (1.05,-0.02) {token $t$};
\draw[arr] (1.05,-0.02) -- (1.05,0.3);
% ============ panel 2: the score, once per token ============
\node[ttl] at (3.05,3.2) {2\;\;Score, once per token};
\node[box,minimum width=15mm] (gB) at (3.95,\yB) {$z\big(\lVert\Delta h_B\rVert\big)$};
\node[box,minimum width=15mm] (gA) at (3.95,\yA) {$z\big(\lVert\Delta h_A\rVert\big)$};
\node[ours,minimum width=20mm] (s) at (5.9,1.45) {$s(t)=z_A-z_B$};
\node[font=\scriptsize,text=mdl,anchor=north] at (5.9,1.18) {fixed at generation};
\node[ours] (h) at (4.9,0.15) {store $h_A$ of the last $w$ tokens\\to recompute their queries};
\draw[earr] (1.65,\yB) -- (gB.west);
\draw[earr] (1.65,\yA) -- (gA.west);
\draw[earr] (2.3,\yA) |- (h.west);
\draw[arr] (gB.east) -- ++(0.15,0) |- ([yshift=2pt]s.west);
\draw[arr] (gA.east) -- ++(0.15,0) |- ([yshift=-2pt]s.west);
% ============ panel 3: compaction ============
\node[ttl] at (7.2,3.2) {3\;\;Compaction};
\node[sub] at (9.5,3.2) {every $\tau$ steps, once the cache exceeds $K$};
\def\ytop{2.05}
\def\ybot{0.3}
\foreach \y in {\ytop,\ybot} {
  \draw[mdl,fill=mdllt,line width=0.3pt] (7.2,\y) rectangle (7.95,\y+0.32);
  \node[font=\scriptsize,text=mdl] at (7.575,\y+0.16) {prompt};
  \draw[mdl,fill=mdllt,line width=0.3pt] (13.1,\y) rectangle (13.85,\y+0.32);
  \node[font=\scriptsize,text=mdl] at (13.475,\y+0.16) {recent};
  \foreach \k in {0,...,3} {\foreach \c in {0,...,7} {\node[cell,fill=white] at (8.08+\k*1.25+\c*0.13,\y) {};}}
}
\foreach \k/\cap in {0/64,1/8,2/32,3/64} {\node[font=\scriptsize,text=mdl] at (8.6+\k*1.25,\ytop-0.17) {cap \cap};}
% the model's recent queries point at a few cached tokens
\foreach \k/\c/\o/\hh in {0/2/13.25/0.92,1/5/13.37/0.76,2/3/13.49/0.6,3/6/13.61/0.46} {
  \draw[epi,line width=0.5pt,->] (\o,\ytop+0.34) .. controls (\o,\ytop+\hh) and (8.145+\k*1.25+\c*0.13,\ytop+\hh) .. (8.145+\k*1.25+\c*0.13,\ytop+0.36);
}
\node[font=\scriptsize,text=epi,anchor=base] at (10.3,2.92) {the last $w$ queries $\cdot$ cached keys $\;\Rightarrow\; r(j)$};
% kept after compaction
\foreach \k/\c in {0/1,0/2,0/4,0/6, 1/5, 2/3,2/7, 3/0,3/3,3/6,3/7} {\node[kept] at (8.08+\k*1.25+\c*0.13,\ybot) {};}
% fill takes the highest r(j) among the evicted, which sit mostly where the tier cut hardest
\foreach \k/\c in {1/2, 1/7, 2/0} {\node[filled] at (8.08+\k*1.25+\c*0.13,\ybot) {};}
\draw[arr,line width=0.6pt] (7.575,\ytop-0.06) -- (7.575,\ybot+0.38);
\node[font=\scriptsize,text=ink,anchor=west,align=left] at (8.0,1.2) {%
  \textbf{tier}: cap each segment by its cached-key variance\\
  \textcolor{epi}{\textbf{rank}: keep the tokens with the highest $r(j)$}\\
  \textcolor{epi}{\textbf{fill}: spend the unused budget by $r(j)$}};
% key for the cache cells
\def\yk{-0.42}
\node[kept] at (8.08,\yk) {};
\node[font=\scriptsize,text=mdl,anchor=west] at (8.24,\yk+0.16) {kept by rank};
\node[filled] at (9.85,\yk) {};
\node[font=\scriptsize,text=mdl,anchor=west] at (10.01,\yk+0.16) {kept by fill};
\node[cell,fill=white] at (11.55,\yk) {};
\node[font=\scriptsize,text=mdl,anchor=west] at (11.71,\yk+0.16) {evicted};
\end{tikzpicture}
\caption{\textbf{\methodname~reads what it needs from the forward pass; the attention matrix
is never formed.} (1)~Decoding runs the unmodified FlashAttention kernel. (2)~Each token gets a
score $s(t)$, fixed at generation, from the hidden-state change at two layers. (3)~Every $\tau$
steps over budget, segments are capped by tier and ranked by $r(j)$, the attention of the last $w$
queries recomputed from Band-A states (\methodseg~ranks by $s(t)$); positions are unchanged.
Blue: what \methodname~adds.}
\vspace{-5mm}
\label{fig:pipeline}
\end{figure}


==> figures/pipeline_v7_contrast.tex <==
% The method figure (bible D-5), redrawn Sep 26 as the paper's argument rather than its plumbing:
% one trace under two policies, the recent queries as the highlighted crux, the outcome drawn.
% Schematic token rows; the words are the model's own from Figure 4 (problem 10). The previous
% mechanism drawing is kept in figures/pipeline_v6_mechanism.tex for the appendix.
\vspace{-1mm}
\begin{figure}[t]
\vspace{-4mm}
\centering
\begin{tikzpicture}[x=1cm,y=1cm,font=\footnotesize,
  >={Stealth[length=1.5mm,width=1.2mm]},
  lab/.style={font=\footnotesize\bfseries,text=ink,anchor=west,inner sep=0},
  sub/.style={font=\scriptsize,text=mdl,anchor=west,inner sep=0,align=left},
  tok/.style={circle,draw=mdl!70,fill=white,line width=0.35pt,minimum size=1.9mm,inner sep=0},
  kept/.style={tok,fill=epimid,draw=epimid},
  filled/.style={tok,pattern=north east lines,pattern color=epi,draw=epi,line width=0.3pt},
  gone/.style={tok,draw=mdl!45,fill=white,line width=0.3pt},
  qry/.style={tok,fill=epi,draw=epi},
  bub/.style={draw=mdl,fill=white,rounded corners=2pt,inner sep=3pt,align=left,font=\scriptsize,text=ink,text width=39mm},
  qarr/.style={->,draw=epi,line width=0.55pt},
  xarr/.style={->,draw=fail,line width=0.55pt,dashed},
]
\def\xz{3.45}\def\dx{0.185}\def\ya{2.35}\def\yb{0.95}
% ---------- row (a): a score fixed when the token was written ----------
\node[lab] at (0,\ya+0.3) {(a) fixed score};
\node[sub] at (0,\ya-0.24) {keeps what looked\\important when written};
\foreach \i in {0,...,33} {\node[gone] (a\i) at (\xz+\i*\dx,\ya) {};}
\foreach \i in {0,1,2,3,4,6,7,10,12,13,16,18,20,23,25,27} {\node[kept] (a\i) at (\xz+\i*\dx,\ya) {};}
\foreach \i in {28,...,33} {\node[qry] (a\i) at (\xz+\i*\dx,\ya) {};}
\draw[xarr] (a30.north) .. controls (\xz+30*\dx,\ya+0.75) and (\xz+9*\dx,\ya+0.75) .. (a9.north);
\draw[xarr] (a32.north) .. controls (\xz+32*\dx,\ya+0.62) and (\xz+15*\dx,\ya+0.62) .. (a15.north);
\draw[xarr] (a33.north) .. controls (\xz+33*\dx,\ya+0.48) and (\xz+22*\dx,\ya+0.48) .. (a22.north);
\foreach \i in {9,15,22} {\node[font=\scriptsize,text=fail,anchor=north,inner sep=1pt] at (\xz+\i*\dx,\ya-0.1) {\xmark};}
\node[bub] (ba) at (11.8,\ya+0.02) {\ldots which is 2220, which is 2220, which is 2220, which is 2220 \ldots\\[1pt]\textcolor{fail}{\xmark~runs to the length cap}};
\draw[->,draw=mdl,line width=0.4pt] (a33.east) -- (ba.west);
% ---------- row (b): the recent queries choose ----------
\node[lab] at (0,\yb+0.3) {(b) \methodname};
\node[sub] at (0,\yb-0.24) {keeps what the recent\\queries point to};
\foreach \i in {0,...,33} {\node[gone] (b\i) at (\xz+\i*\dx,\yb) {};}
\foreach \i in {0,1,2,3,6,9,12,15,17,19,22,24,26} {\node[kept] (b\i) at (\xz+\i*\dx,\yb) {};}
\foreach \i in {5,11,21} {\node[filled] (b\i) at (\xz+\i*\dx,\yb) {};}
\foreach \i in {28,...,33} {\node[qry] (b\i) at (\xz+\i*\dx,\yb) {};}
\draw[qarr] (b30.north) .. controls (\xz+30*\dx,\yb+0.75) and (\xz+9*\dx,\yb+0.75) .. (b9.north);
\draw[qarr] (b32.north) .. controls (\xz+32*\dx,\yb+0.62) and (\xz+15*\dx,\yb+0.62) .. (b15.north);
\draw[qarr] (b33.north) .. controls (\xz+33*\dx,\yb+0.48) and (\xz+22*\dx,\yb+0.48) .. (b22.north);
\foreach \i in {9,15,22} {\node[font=\scriptsize,text=epi,anchor=north,inner sep=1pt] at (\xz+\i*\dx,\yb-0.1) {\cmark};}
\node[bub] (bb) at (11.8,\yb+0.02) {Thus, the smallest number that meets the criteria is 2220. \texttt{\textbackslash boxed\{2220\}}\\[1pt]\textcolor{epi}{\cmark~stops}};
\draw[->,draw=mdl,line width=0.4pt] (b33.east) -- (bb.west);
% ---------- shared annotations ----------
\draw[epi,line width=0.4pt] (\xz+28*\dx-0.1,\ya+0.78) -- (\xz+28*\dx-0.1,\ya+0.86) -- (\xz+33*\dx+0.1,\ya+0.86) -- (\xz+33*\dx+0.1,\ya+0.78);
\node[font=\scriptsize,text=epi,anchor=south] at (\xz+30.5*\dx,\ya+0.86) {the last $w$ queries};
\node[font=\scriptsize,text=mdl,anchor=east,inner sep=1pt] at (\xz-0.14,\ya) {prompt};
\node[font=\scriptsize,text=mdl,anchor=east,inner sep=1pt] at (\xz-0.14,\yb) {prompt};
% ---------- legend and the rule ----------
\def\yl{-0.05}
\node[kept] at (3.45,\yl) {};      \node[sub,anchor=west] at (3.6,\yl) {kept by rank};
\node[filled] at (5.3,\yl) {};   \node[sub,anchor=west] at (5.45,\yl) {kept by fill};
\node[gone] at (7.05,\yl) {};      \node[sub,anchor=west] at (7.2,\yl) {evicted};
\node[qry] at (8.4,\yl) {};      \node[sub,anchor=west] at (8.55,\yl) {recent queries};
\node[sub,anchor=north west,text width=138mm] at (0,\yl-0.2) {%
  Every $\tau$ steps, once the cache exceeds $K$: tier each 128-slot segment by the variance of its cached
  keys, rank within it by $r(j)$, the attention of the last $w$ queries recomputed from stored Band-A
  hidden states against the cached keys, and fill the unused budget by $r(j)$. \methodseg~ranks by the
  fixed score $s(t)$ instead. The attention matrix is never formed; positions are unchanged.};
\end{tikzpicture}
\caption{\textbf{What eviction keeps decides whether the model can stop.} One trace under two
policies, schematically; the words are the model's own (Figure~\ref{fig:loop}). (a)~A score fixed
when each token is generated keeps the tokens that looked important then; the model's recent
queries (blue) point at tokens that are gone, and it restates the answer until the cap.
(b)~\methodname~recomputes those queries from the hidden states it stored and keeps the tokens
they point to; the model checks the answer and stops.}
\vspace{-5mm}
\label{fig:pipeline}
\end{figure}

